Fault Diagnosability Analysis of Multi-Mode Systems

Multi-mode systems can operate in different modes, leading to large numbers of different dynamics. Consequently, applying traditional structural diagnostics to such systems is often untractable. To address this challenge, we present a multi-mode diagnostics algorithm that relies on a multi-mode extension of the Dulmage-Mendelsohn decomposition. We introduce two methodologies for modeling faults, either as signals or as Boolean variables, and apply them to a modular switched battery system in order to demonstrate their effectiveness and discuss their respective advantages.

==> Background.tex <==
\section{Background}

\subsection{Multi-mode DAE}
\textcolor{red}{France part}

\subsection{Diagnostics}
General definitions of diagnostics.
\begin{description}
	\item[Detectability] ...
\end{description}

\begin{description}
	\item[Isolability] ...
\end{description}


\begin{description}
	\item[Isolability Matrix] The interpretation of the matrix is that $f_i$ is isolable from $f_j$
	in mode $m$ if the expression in position $(f_i, f_j)$ evaluates to
	true in mode $m$. The NF-column indicates which faults that
	are detectable.
\end{description}
 
\subsubsection{Extended Dulmage-Mendelsohn decomposition}
talk about the original one and the extended one that we use for diagnostics.

\begin{description}
	\item[Dulmage-Mendelsohn (DM) decomposition] ...
\end{description}

\begin{description}
	\item[Extended (DM) decomposition] \cite{Extended-DM}...
\end{description}

Mention that the extended one, eventhough it works for isolability in single mode systems,
however, it does not work for multi-mode systems, and in MM systems we need to have as many
 as mode, DMs. And this is the motivation for this work! which we explain the importance of that in the next section.

==> Multi-mode_diagnosability1.tex <==
\section{Multi-mode diagnosability1}

	Given a model $M$ of equations $E$. There are Boolean variables $F = (F_1, F_2, \ldots, F_n)$ such that $F_i = \ttrue$ if a fault $i$ is present and $\ffalse$ otherwise. There are Boolean variables $S = (S_1, \ldots, S_n)$ that represent system mode switches, such as valves and switches.

As The multi-mode Dulmage-Mendelsohn decomposition computes for each equation $e$ in a model $M$ a Boolean expression 
\begin{equation}
	e^+(f,s) = 
	\begin{cases}
		1 & \text{if $e \in M^+$ }\\
		0 & \text{otherwise.}
	\end{cases}
\end{equation}  
These functions will be used to answer detectability and isolability questions in the following sections. These Boolean functions can become large. Therefore, they are implemented as BDDs. 

\subsubsection{Example}

\begin{align*}
	e_{\texttt{f\_cell}}^+ = \lnot \ba \land \lnot \texttt{f\_cell} \land \lnot \texttt{f\_i} \land \lnot \texttt{f\_v} \lor \\
	\lnot \texttt{forward} \land \lnot \texttt{f\_cell} \land \lnot \texttt{f\_i} \land \lnot \texttt{f\_v} \lor \\
	\lnot \texttt{forward} \land \lnot \texttt{backward} \land \lnot \texttt{f\_cell} \land \lnot \texttt{f\_v}
\end{align*}

\begin{align*}
	e_{\texttt{f\_cell}}^+ = \lnot \texttt{backward} \lor
	\lnot \texttt{forward} 
\end{align*}

\begin{align*}
	e_{\texttt{f\_cell}}^+(\texttt{f\_i}) = \lnot \texttt{backward} \land
	\lnot \texttt{forward} 
\end{align*}

\begin{align*}
	e_{\texttt{f\_cell}}^+(M\backslash \{e_{\texttt{f\_i}}\}) = \lnot \texttt{backward} \land
	\lnot \texttt{forward} 
\end{align*}



A model is a set of equations $M$ a set of unknown real variables $X$ a set of Boolean variables   
\begin{center}
	\begin{tabular}{l|cc}
		& \multicolumn{2}{c}{\texttt{backward}} \\
		\texttt{forward} & 0 & 1\\ \hline
		0 & \texttt{bypass} & \texttt{backward}\\ 
		1 & \texttt{forward}  & \texttt{invalid}\\
	\end{tabular}
\end{center}
\subsection{Detectability Analysis}

From single to multiple mode formulation.

A fault $f$ is detectable in system $M$ if 
\begin{equation}
	\{\neg f\} \cup \{e_f^+\} \not \models \emptyset
\end{equation}
is consistent. Since $e_f^+ \models \neg f$ it is sufficient to check if 
\begin{equation}
	\{e_f^+\} \not \models \emptyset
\end{equation} 
This means that there exists at least one mode assignment such that $e_f^+$ is true.

Consider the one SM-battery example and the BDD representation of $e^+$. 

In the example $\texttt{f\_cell}$ is detectable in the modes $$\exists f. e_{\texttt{f\_cell}}^+(f,s) = \lnot \texttt{backward} \land
\lnot \texttt{forward}$$


\subsubsection{Isolability Analysis}


A fault $f_i$ is isolable from $f_j$ in system $M$ if 
\begin{equation}
	\{\neg f_i, f_j\} \cup \{e_{f_i}^+\} \not \models \emptyset
\end{equation}
is consistent.

In the example 
\begin{align*}
	\{\neg \texttt{f\_cell}, \texttt{f\_i}\} \cup \{e_{\texttt{f\_cell}}^+\} = 
	\lnot \texttt{forward} \land \lnot \texttt{backward} \land \lnot \texttt{f\_v}
\end{align*}
This formula tells that $\texttt{f\_cell}$ is isolable from $\texttt{f\_i}$ if and only if the submodule is in \texttt{bypass} mode and the voltage sensor is okey. This is easily extended to multiple fault isolability analysis. If we would like to compute if fault $\texttt{f\_cell}$ is isolable from the double fault including $\texttt{f\_i}$ and $\texttt{f\_v}$ the query would be
\begin{align*}
	\{\neg \texttt{f\_cell}, \texttt{f\_i},\texttt{f\_v}\} \cup \{e_{\texttt{f\_cell}}^+\} = \emptyset
\end{align*}
Since no valuation is consistent it follows that $\texttt{f\_cell}$ is not isolable from the double fault.




Single fault isolability
Multiple fault isolability


The term "always detectable/isolable" indicates that the specified fault is detectable/isolable across all mode assignments.
The equation set $ (M\backslash{e_{f_j}})^+ $ in structural isolability definition is obtained by eliminating one equation, i.e., $e_{f_j}$, and subsequently calculating the over-determined component.
\begin{itemize}
	\item LiU part with the description of how the code work:
	\begin{itemize}
		\item Detectability: 
		\item Isolability: how to check it based on MMDM
		\item Show the algorithm by a function
		\item Show an Isolability matrix for one cell (or for the example)
		and explain how it works. With complete expressions
		\item Say that we use BDD representation to handle the large expressions, and also reference the package used.  The BDD package is available on~\cite{tulipcontrol}.
	\end{itemize}
\end{itemize}

The main targets at hand is determining if it is possible to isolate the faults $ (f_i, f_j)$ in different operational modes of a multi-mode system. In an isolability matrix, the presence of the entry "1" at the intersection of $ (f_i, f_j)$ signifies that fault $ (f_i)$ can be isolated from fault $ (f_j)$. Two prospective situations come to light: firstly, faults are isolable across all modes, denoted as "always isolable"; secondly, this isolation occurs in at least one mode. In the latter instance, the objective is to identify the optimal mode, considering factors such as availability, safety, and related criteria.



==> Multi-mode_diagnosability2.tex <==
\section{Multi-mode diagnosability}

\currentstatus{After notation change}

\requiredactions{Ready for proofreading}

Multi-mode diagnosability analyses of the two methodologies explained in Section~\ref{sec:mmsystems} will be addressed. Subsequently, an evaluation of the advantages and disadvantages of each approach will be given. 

\subsection{Diagnosability} 
The main problem addressed will be to compute the detectability and single fault isolability of a multi-mode model with the set of single faults $F$ either modeled as fault signals or Boolean variables. 
For a single-mode system and in the context of structural analysis, diagnosability analysis is performed by computing fault detectability of all faults $f\in F$ and fault isolability for all fault pair $(f_i,f_j)\in F\times F$. Note in Definition~\ref{def:str_det} that detectability of a fault $f$ can be seen as a special case of isolating $f$ from the empty set of faults, i.e., the no-fault case \texttt{NF}. Then the detectability and isolability of a model can compactly be described by the diagnosability $D$ defined in the following way
\begin{align*}
	D_{(f, \texttt{NF})} &= \ttrue \text{ if } f \text{ is detectable} \\ 
	D_{(f_i, f_j)} &= \ttrue \text{ if } (f_i,f_j) \in F\times F \text{ is isolable}
\end{align*}
For a multi-mode model, $D_{(f_i, f_j)}$ are Boolean functions $\mathbb{M} \rightarrow \bool$ for all $f_i\in F$ and $f_j\in F \cup \{\texttt{NF}\}$ that should be computed in diagnosability analysis.
 
\subsection{Diagnosability based on the fault signal approach}

In the fault signal approach, a multi-mode model $\Ms$ with a set of faults $F$ is described by its corresponding fault signals $f = (f_1, f_2, \ldots, f_n)$ such that $f_i \neq 0$ if fault $i$ is present and $f_i = 0$ otherwise. There are Boolean variables called system mode variables denoted by $S = (S_1, \ldots, S_n)$ which represent, e.g., valves and switch positions in the system. It is assumed that faults are introduced in equations without system mode variables. In the model of an SM the system mode variables are $\forw$ and $\back$ according to Table~\ref{tab:SMswmodes}. 



For each equation $e \in E$ in a model $\Ms$, {\mmDM} returns a Boolean expression dependent on the mode variables, i.e., $\eover{e} : \mathbb{M}_s \rightarrow \bool$, where the superscript $+$ denotes the over-determined part. These functions will be used to answer detectability and isolability questions. The \texttt{dd} library (see ~\cite{tulip-control:dd}) is used for efficiently handling these functions as BDDs.
	
	
\begin{definition}[Structural detectability]
	A fault $f_i$ is structurally detectable in a multi-mode system $\Ms$ if 
	\begin{equation}
		\eover{e_{f_i}}(\Ms) \not \equiv \ffalse, 
	\end{equation}
	where $e_{f_i}$ is the equation including the fault $f_i$. $\blacklozenge$
\end{definition}
This means that a fault is structurally detectable if there exists at least one valid mode assignment $S=S_0$ such that $\eover{e_{f_i}}(\Ms)[S:=S_0] = \ttrue$. It is also possible to compute the detectability of $f_i$ in a specific mode $S=S_0$ by evaluating if $\eover{e_{f_i}}(\Ms)[S:=S_0]$ is true. Furthermore, a fault $f$ is detectable in all (valid) modes if 
\begin{equation}
	\texttt{invariant} \rightarrow \eover{e_{f}}(\Ms)
\end{equation}
Consider a system with only one SM defined in Section~\ref{sec:mmsystems} and the fault $\texttt{f\_cell}$. This fault is detectable for the modes defined by $\eover{e_{f_{cell}}}(\Ms) = \lnot \texttt{backward} \lor \lnot \texttt{forward}$, that is equivalent to the invariant, which implies that the $\texttt{f\_cell}$ is detectable in all modes. 	

Algorithm~\ref{alg:mmdetectability} computes the fault detectability of all faults in a model $\Ms$. On row~\ref{row:always-det} the Boolean expression is simplified for faults that are detectable in all valid modes. Note that only one $\texttt{mmDM}$ is performed to compute the detectability of all faults in all modes. This algorithm will be used when computing fault isolability presented next.
\begin{algorithm}
	\caption{$\langle D_{(f,\texttt{NF})} \rangle_{f\in F} = \text{Detectability}(\Ms)$
	}\label{alg:mmdetectability}
	\begin{algorithmic}[1] %
	\State $\langle \eover{e}(\Ms) \rangle_{e\in E} = \texttt{mmDM}(\Ms)$
	\ForAll{$f \in F$}		
		\If{$\texttt{invariant}\rightarrow \eover{e_f}(\Ms) $}
			\State $D_{(f,\texttt{NF})} = \ttrue$ \Comment{Detectable in all valid modes} \label{row:always-det}
		\Else 	
			\State $D_{(f,\texttt{NF})} = \eover{e_{f}}(\Ms)$
		\EndIf
	\EndFor		
	\end{algorithmic}
\end{algorithm}
	
		

	
\begin{definition}[Structural isolability]
	A fault $f_i$ is structurally isolable from $f_j$ in a multi-mode system $\Ms$ if 
	\begin{equation}
		\eover{e_{f_i}}(\Ms \backslash \{e_{f_j}\}) \not \equiv \ffalse 
	\end{equation}
	where $\Ms \backslash \{e_{f_j}\}$ is obtained by removing equation $e_{f_j}$ from the model $\Ms$. $\blacklozenge$
\end{definition}

As an illustration, considering one SM, the formula
\begin{equation*}
	\eover{e_{f_\text{cell}}}(\Ms \backslash \{e_{f_{i_\text{cell}}}\}) = \lnot \texttt{backward} \land \lnot \texttt{forward},
\end{equation*} 
shows that $f_\text{cell}$ is isolable from $f_{i_\text{cell}}$  
only in the bypass modes according to Table~\ref{tab:SMswmodes}.
		
Algorithm~\ref{alg:mmiso} computes the multi-mode diagnosability $D$ including both detectability and isolability of a mult-mode model $\Ms$, with the assistance of the {\mmDM} defined in Section~\ref{sec:mmdm} and Algorithm~\ref{alg:mmdetectability}. 
It is without loss of generality assumed that there is at most one fault in each equation.
		
\begin{algorithm}
	\caption{$D = \text{Diagnosability}(\Ms)$}\label{alg:mmiso}
	\begin{algorithmic}[1] %
	\State $\langle D_{(f,\texttt{NF})} \rangle_{f\in F} = \text{Detectability}(\Ms)$
	\ForAll{$f \in F$}
		\If{$f$ is detectable}
			\State $\langle D_{(f_i,f)} \rangle_{f_i\in F} = \text{Detectability}(\Ms\setminus \{e_{f}\})$
		\Else \Comment{Avoid unnecessary \texttt{mmDM}}
			\State $\langle D_{(f_i,f)} \rangle_{f_i\in F} = \langle D_{(f_i,\texttt{NF})} \rangle_{f_i\in F}$  					
		\EndIf
	\EndFor
	\end{algorithmic}
\end{algorithm}
	
The diagnosability result of Algorithm~\ref{alg:mmiso}, applied to the one SM example is shown in Table~\ref{tab:1SM_iso_matrix}. The first column $\texttt{NF}$ indicates that all faults are detectable in all modes. The 2 by 2 block of $\ffalse$:s indicates that the faults $f_\text{cell}$ and $f_{v_\text{cell}}$ are not isolable in any mode. The entries with $\by$ indicates that the faults $f_\text{cell}$ and $f_{v_\text{cell}}$ are isolable from fault $f_{i_\text{cell}}$ in bypass mode.
		
\begin{table}[h]
	\centering
	\caption{Multi-mode fault diagnosability matrix for the one SM example.}
	\vspace*{-2mm}
	\label{tab:1SM_iso_matrix}
	\begin{tabular}{c|cccc}
		\hline 
		& $ \verb|NF| $  & $ \verb|f_cell| $  & $ \verb|f_v_cell| $ & $ \verb|f_i_cell| $  \\
		\hline
		$ \verb|f_cell| $   & \cellcolor{lightgray} $\ttrue$ & $\ffalse$ & $\ffalse$  & $\by$ \\
			
		$ \verb|f_v_cell| $ & \cellcolor{lightgray} $\ttrue$ &  $\ffalse$  &  $\ffalse$ & $\by$ \\
				
		$ \verb|f_i_cell| $ & \cellcolor{lightgray} $\ttrue$ &  $\by$  & $\by$ &  $\ffalse$ \\ %
		\hline
	\end{tabular}
\end{table}


\subsection{Diagnosability based on the Boolean fault approach}
	
	In this approach, faults are defined as Boolean mode variables $F = (F_1, F_2, \ldots, F_n)$ such that $F_i \equiv \ttrue$ if a fault $i$ is present and $F_i \equiv \ffalse$ otherwise. As in the preceding approach, $S$ is the set of Boolean variables that represent system modes.
	The {\mmDM} decomposition computes, for each equation $e \in E$, a Boolean function dependent on the mode variables $F$ and $S$, i.e., $\eover{e} : \mathbb{\MB} \rightarrow \bool$.
 Similar to the previous methodology, the superscript `+' denotes the over-determined part of DM, and the present approach similarly employs this function to assess the diagnosability of multi-mode systems. However, in contrast to the preceding methodology, it is notable that the {\mmDM} in this context is a function of both system modes and faults.
	\subsubsection{Detectability Analysis}
	  \begin{definition} [Structural detectability]
	  	Let $\mathcal{F}$ be the set of faults in a multi-mode system $\MB$. A fault $F_i \in  \mathcal{F}$ is structurally detectable if 
	  	%
	  		%
	  		%
	  	\begin{equation}
	  		\eover{e_{F_{i}}}(\MB)[F := \ffalse] \not \equiv \ffalse,
	  	\end{equation}
	  	%
	  		%
	  		%
	  		%
	  	where $e_{F_i}$ is the equation related to the fault $F_i$. $\blacklozenge$
	  \end{definition}      
		
	Consider the one SM-battery example and the BDD representation of $\eover{}$. 
	In the example $\texttt{F\_cell}$ is detectable in the modes 
	\begin{align*}
		&\eover{e_{F_{i_{cell}}}}(\MB)[F_{cell}, F_{i_{cell}}, F_{v_{cell}}:= \ffalse] =\\
		&(\lnot \ba \land \lnot \texttt{F\_cell} \land \lnot \texttt{F\_i\_cell} \land \lnot \texttt{F\_v\_cell}) \lor \\
		&(\lnot \texttt{forward} \land \lnot \texttt{F\_cell} \land \lnot \texttt{F\_i\_cell} \land \lnot \texttt{F\_v\_cell}) \lor \\
		&(\lnot \texttt{forward} \land \lnot \texttt{backward} \land \lnot \texttt{F\_cell} \land \lnot \texttt{F\_v\_cell}).
	\end{align*}
	The implication here is that in modes $\forw$ and $\back$, the fault $\texttt{F\_cell}$ is detectable if and only if the voltage and current sensors are not-faulty/okay. However, in the $\by$ mode, the criterion for the detectability of $\texttt{F\_cell}$ is the voltage sensor is not-faulty/okay.
	
	\subsubsection{Isolability Analysis}
	
	 \begin{definition}[Single fault structural isolability]
	 	A single fault $F_i $ is structural isolable from single $F_j$ in multi-mode system $\MB$ if 
	 	%
	 		%
	 		%
	 	\begin{equation}
	 		\eover{e_{F_{i}}}(\MB)[ F_j:= \ttrue, F_k: {k\neq j} := \ffalse] \not \equiv \ffalse,
	 	\end{equation}
	 	is satisfiable. $\blacklozenge$ 
	 \end{definition}
	In the one SM example 
	\begin{align*}
		&\eover{e_{F_{cell}}}(\MB)[F_{i_{cell}}:= \ttrue, F_{cell}, F_{v_{cell}}:= \ffalse] =\\
		&\lnot \texttt{forward} \land \lnot \texttt{backward}.
	\end{align*}This formula tells that $\texttt{F\_cell}$ is isolable from $\texttt{F\_i\_cell}$ if and only if the submodule is in $\by$ mode, yielding an outcome consistent with the example in the preceding methodology. The concept of isolability can easily be extended to multiple fault isolability analysis as the following.
	\begin{definition}[Multiple fault structural isolability]
		Let $\mathcal{F}$ be the set of faults and $\Gamma \subseteq \mathcal{F}$ represents a multiple fault set, then $F_i \in \mathcal{F}$ is structural isolable from multiple fault $\Gamma$ if
		\begin{equation}
			\eover{e_{F_i}}(\MB)[\Gamma := \ttrue, {\tilde{F} \in (\mathcal{F}\backslash \Gamma)} := \ffalse] \not \equiv \ffalse,
		\end{equation}
		is satisfiable. $\blacklozenge$
	\end{definition}
	 In the event that one intends to determine the isolability of fault $\texttt{F\_cell}$ from the dual fault scenario including both $\texttt{F\_i\_cell}$ and $\texttt{F\_v\_cell}$ the corresponding query would be formulated as follows
	\begin{equation}
		\eover{e_{F_{cell}}}(\MB)[F_{cell} := \ffalse, F_{i_{cell}}, F_{v_{cell}} := \ttrue] \equiv \ffalse.
	\end{equation}
	Since no valuation is consistent it follows that $\texttt{F\_cell}$ is not isolable from the double fault.



In order to verify the effectiveness of these algorithms, we use them on a case study in the next section.

	
	







